Observation of the decay $\chi_{cJ} \to \Omega^- \bar{\Omega}^+$

Using an $e^+e^-$ collision data sample of $(27.08 \pm 0.14) \times 10^{8}$ $\psi(3686)$ events collected by the BESIII detector, we report the first observation of $\chi_{cJ} \to \Omega^- \bar{\Omega}^+$ ($J=0,\,1,\,2$) decays with significances of $5.6\sigma$, $6.4\sigma$, and $18\sigma$, respectively, where the $\chi_{cJ}$ mesons are produced in the radiative $\psi(3686)$ decays. The branching fractions are determined to be $\mathcal{B}(\chi_{c0} \to \Omega^- \bar{\Omega}^+) = (3.51 \pm 0.54 \pm 0.29) \times 10^{-5}$, $\mathcal{B}(\chi_{c1} \to \Omega^- \bar{\Omega}^+) = (1.49 \pm 0.23 \pm 0.10) \times 10^{-5}$, and $\mathcal{B}(\chi_{c2} \to \Omega^- \bar{\Omega}^+) = (4.52 \pm 0.24 \pm 0.18) \times 10^{-5}$, where the first and second uncertainties are statistical and systematic, respectively.

==> arXivAuthorlist/authorlist_2022-10-24.tex <==
%% Saved at => 2022-10-24
{\small M.~Ablikim$^{1}$, M.~N.~Achasov$^{13,b}$, P.~Adlarson$^{73}$, R.~Aliberti$^{34}$, A.~Amoroso$^{72A,72C}$, M.~R.~An$^{38}$, Q.~An$^{69,56}$, Y.~Bai$^{55}$, O.~Bakina$^{35}$, I.~Balossino$^{29A}$, Y.~Ban$^{45,g}$, V.~Batozskaya$^{1,43}$, K.~Begzsuren$^{31}$, N.~Berger$^{34}$, M.~Bertani$^{28A}$, D.~Bettoni$^{29A}$, F.~Bianchi$^{72A,72C}$, E.~Bianco$^{72A,72C}$, J.~Bloms$^{66}$, A.~Bortone$^{72A,72C}$, I.~Boyko$^{35}$, R.~A.~Briere$^{5}$, A.~Brueggemann$^{66}$, H.~Cai$^{74}$, X.~Cai$^{1,56}$, A.~Calcaterra$^{28A}$, G.~F.~Cao$^{1,61}$, N.~Cao$^{1,61}$, S.~A.~Cetin$^{60A}$, J.~F.~Chang$^{1,56}$, T.~T.~Chang$^{75}$, W.~L.~Chang$^{1,61}$, G.~R.~Che$^{42}$, G.~Chelkov$^{35,a}$, C.~Chen$^{42}$, Chao~Chen$^{53}$, G.~Chen$^{1}$, H.~S.~Chen$^{1,61}$, M.~L.~Chen$^{1,56,61}$, S.~J.~Chen$^{41}$, S.~M.~Chen$^{59}$, T.~Chen$^{1,61}$, X.~R.~Chen$^{30,61}$, X.~T.~Chen$^{1,61}$, Y.~B.~Chen$^{1,56}$, Y.~Q.~Chen$^{33}$, Z.~J.~Chen$^{25,h}$, W.~S.~Cheng$^{72C}$, S.~K.~Choi$^{10A}$, X.~Chu$^{42}$, G.~Cibinetto$^{29A}$, S.~C.~Coen$^{4}$, F.~Cossio$^{72C}$, J.~J.~Cui$^{48}$, H.~L.~Dai$^{1,56}$, J.~P.~Dai$^{77}$, A.~Dbeyssi$^{19}$, R.~ E.~de Boer$^{4}$, D.~Dedovich$^{35}$, Z.~Y.~Deng$^{1}$, A.~Denig$^{34}$, I.~Denysenko$^{35}$, M.~Destefanis$^{72A,72C}$, F.~De~Mori$^{72A,72C}$, B.~Ding$^{64,1}$, X.~X.~Ding$^{45,g}$, Y.~Ding$^{33}$, Y.~Ding$^{39}$, J.~Dong$^{1,56}$, L.~Y.~Dong$^{1,61}$, M.~Y.~Dong$^{1,56,61}$, X.~Dong$^{74}$, S.~X.~Du$^{79}$, Z.~H.~Duan$^{41}$, P.~Egorov$^{35,a}$, Y.~L.~Fan$^{74}$, J.~Fang$^{1,56}$, S.~S.~Fang$^{1,61}$, W.~X.~Fang$^{1}$, Y.~Fang$^{1}$, R.~Farinelli$^{29A}$, L.~Fava$^{72B,72C}$, F.~Feldbauer$^{4}$, G.~Felici$^{28A}$, C.~Q.~Feng$^{69,56}$, J.~H.~Feng$^{57}$, K~Fischer$^{67}$, M.~Fritsch$^{4}$, C.~Fritzsch$^{66}$, C.~D.~Fu$^{1}$, Y.~W.~Fu$^{1}$, H.~Gao$^{61}$, Y.~N.~Gao$^{45,g}$, Yang~Gao$^{69,56}$, S.~Garbolino$^{72C}$, I.~Garzia$^{29A,29B}$, P.~T.~Ge$^{74}$, Z.~W.~Ge$^{41}$, C.~Geng$^{57}$, E.~M.~Gersabeck$^{65}$, A~Gilman$^{67}$, K.~Goetzen$^{14}$, L.~Gong$^{39}$, W.~X.~Gong$^{1,56}$, W.~Gradl$^{34}$, S.~Gramigna$^{29A,29B}$, M.~Greco$^{72A,72C}$, M.~H.~Gu$^{1,56}$, Y.~T.~Gu$^{16}$, C.~Y~Guan$^{1,61}$, Z.~L.~Guan$^{22}$, A.~Q.~Guo$^{30,61}$, L.~B.~Guo$^{40}$, R.~P.~Guo$^{47}$, Y.~P.~Guo$^{12,f}$, A.~Guskov$^{35,a}$, X.~T.~H.$^{1,61}$, W.~Y.~Han$^{38}$, X.~Q.~Hao$^{20}$, F.~A.~Harris$^{63}$, K.~K.~He$^{53}$, K.~L.~He$^{1,61}$, F.~H.~Heinsius$^{4}$, C.~H.~Heinz$^{34}$, Y.~K.~Heng$^{1,56,61}$, C.~Herold$^{58}$, T.~Holtmann$^{4}$, P.~C.~Hong$^{12,f}$, G.~Y.~Hou$^{1,61}$, Y.~R.~Hou$^{61}$, Z.~L.~Hou$^{1}$, H.~M.~Hu$^{1,61}$, J.~F.~Hu$^{54,i}$, T.~Hu$^{1,56,61}$, Y.~Hu$^{1}$, G.~S.~Huang$^{69,56}$, K.~X.~Huang$^{57}$, L.~Q.~Huang$^{30,61}$, X.~T.~Huang$^{48}$, Y.~P.~Huang$^{1}$, T.~Hussain$^{71}$, N~H\"usken$^{27,34}$, W.~Imoehl$^{27}$, M.~Irshad$^{69,56}$, J.~Jackson$^{27}$, S.~Jaeger$^{4}$, S.~Janchiv$^{31}$, J.~H.~Jeong$^{10A}$, Q.~Ji$^{1}$, Q.~P.~Ji$^{20}$, X.~B.~Ji$^{1,61}$, X.~L.~Ji$^{1,56}$, Y.~Y.~Ji$^{48}$, Z.~K.~Jia$^{69,56}$, P.~C.~Jiang$^{45,g}$, S.~S.~Jiang$^{38}$, T.~J.~Jiang$^{17}$, X.~S.~Jiang$^{1,56,61}$, Y.~Jiang$^{61}$, J.~B.~Jiao$^{48}$, Z.~Jiao$^{23}$, S.~Jin$^{41}$, Y.~Jin$^{64}$, M.~Q.~Jing$^{1,61}$, T.~Johansson$^{73}$, X.~K.$^{1}$, S.~Kabana$^{32}$, N.~Kalantar-Nayestanaki$^{62}$, X.~L.~Kang$^{9}$, X.~S.~Kang$^{39}$, R.~Kappert$^{62}$, M.~Kavatsyuk$^{62}$, B.~C.~Ke$^{79}$, A.~Khoukaz$^{66}$, R.~Kiuchi$^{1}$, R.~Kliemt$^{14}$, L.~Koch$^{36}$, O.~B.~Kolcu$^{60A}$, B.~Kopf$^{4}$, M.~Kuessner$^{4}$, A.~Kupsc$^{43,73}$, W.~K\"uhn$^{36}$, J.~J.~Lane$^{65}$, J.~S.~Lange$^{36}$, P. ~Larin$^{19}$, A.~Lavania$^{26}$, L.~Lavezzi$^{72A,72C}$, T.~T.~Lei$^{69,k}$, Z.~H.~Lei$^{69,56}$, H.~Leithoff$^{34}$, M.~Lellmann$^{34}$, T.~Lenz$^{34}$, C.~Li$^{42}$, C.~Li$^{46}$, C.~H.~Li$^{38}$, Cheng~Li$^{69,56}$, D.~M.~Li$^{79}$, F.~Li$^{1,56}$, G.~Li$^{1}$, H.~Li$^{69,56}$, H.~B.~Li$^{1,61}$, H.~J.~Li$^{20}$, H.~N.~Li$^{54,i}$, Hui~Li$^{42}$, J.~R.~Li$^{59}$, J.~S.~Li$^{57}$, J.~W.~Li$^{48}$, Ke~Li$^{1}$, L.~J~Li$^{1,61}$, L.~K.~Li$^{1}$, Lei~Li$^{3}$, M.~H.~Li$^{42}$, P.~R.~Li$^{37,j,k}$, S.~X.~Li$^{12}$, T. ~Li$^{48}$, W.~D.~Li$^{1,61}$, W.~G.~Li$^{1}$, X.~H.~Li$^{69,56}$, X.~L.~Li$^{48}$, Xiaoyu~Li$^{1,61}$, Y.~G.~Li$^{45,g}$, Z.~J.~Li$^{57}$, Z.~X.~Li$^{16}$, Z.~Y.~Li$^{57}$, C.~Liang$^{41}$, H.~Liang$^{69,56}$, H.~Liang$^{1,61}$, H.~Liang$^{33}$, Y.~F.~Liang$^{52}$, Y.~T.~Liang$^{30,61}$, G.~R.~Liao$^{15}$, L.~Z.~Liao$^{48}$, J.~Libby$^{26}$, A. ~Limphirat$^{58}$, D.~X.~Lin$^{30,61}$, T.~Lin$^{1}$, B.~J.~Liu$^{1}$, B.~X.~Liu$^{74}$, C.~Liu$^{33}$, C.~X.~Liu$^{1}$, D.~~Liu$^{19,69}$, F.~H.~Liu$^{51}$, Fang~Liu$^{1}$, Feng~Liu$^{6}$, G.~M.~Liu$^{54,i}$, H.~Liu$^{37,j,k}$, H.~B.~Liu$^{16}$, H.~M.~Liu$^{1,61}$, Huanhuan~Liu$^{1}$, Huihui~Liu$^{21}$, J.~B.~Liu$^{69,56}$, J.~L.~Liu$^{70}$, J.~Y.~Liu$^{1,61}$, K.~Liu$^{1}$, K.~Y.~Liu$^{39}$, Ke~Liu$^{22}$, L.~Liu$^{69,56}$, L.~C.~Liu$^{42}$, Lu~Liu$^{42}$, M.~H.~Liu$^{12,f}$, P.~L.~Liu$^{1}$, Q.~Liu$^{61}$, S.~B.~Liu$^{69,56}$, T.~Liu$^{12,f}$, W.~K.~Liu$^{42}$, W.~M.~Liu$^{69,56}$, X.~Liu$^{37,j,k}$, Y.~Liu$^{37,j,k}$, Y.~B.~Liu$^{42}$, Z.~A.~Liu$^{1,56,61}$, Z.~Q.~Liu$^{48}$, X.~C.~Lou$^{1,56,61}$, F.~X.~Lu$^{57}$, H.~J.~Lu$^{23}$, J.~G.~Lu$^{1,56}$, X.~L.~Lu$^{1}$, Y.~Lu$^{7}$, Y.~P.~Lu$^{1,56}$, Z.~H.~Lu$^{1,61}$, C.~L.~Luo$^{40}$, M.~X.~Luo$^{78}$, T.~Luo$^{12,f}$, X.~L.~Luo$^{1,56}$, X.~R.~Lyu$^{61}$, Y.~F.~Lyu$^{42}$, F.~C.~Ma$^{39}$, H.~L.~Ma$^{1}$, J.~L.~Ma$^{1,61}$, L.~L.~Ma$^{48}$, M.~M.~Ma$^{1,61}$, Q.~M.~Ma$^{1}$, R.~Q.~Ma$^{1,61}$, R.~T.~Ma$^{61}$, X.~Y.~Ma$^{1,56}$, Y.~Ma$^{45,g}$, F.~E.~Maas$^{19}$, M.~Maggiora$^{72A,72C}$, S.~Maldaner$^{4}$, S.~Malde$^{67}$, A.~Mangoni$^{28B}$, Y.~J.~Mao$^{45,g}$, Z.~P.~Mao$^{1}$, S.~Marcello$^{72A,72C}$, Z.~X.~Meng$^{64}$, J.~G.~Messchendorp$^{14,62}$, G.~Mezzadri$^{29A}$, H.~Miao$^{1,61}$, T.~J.~Min$^{41}$, R.~E.~Mitchell$^{27}$, X.~H.~Mo$^{1,56,61}$, N.~Yu.~Muchnoi$^{13,b}$, Y.~Nefedov$^{35}$, F.~Nerling$^{19,d}$, I.~B.~Nikolaev$^{13,b}$, Z.~Ning$^{1,56}$, S.~Nisar$^{11,l}$, Y.~Niu $^{48}$, S.~L.~Olsen$^{61}$, Q.~Ouyang$^{1,56,61}$, S.~Pacetti$^{28B,28C}$, X.~Pan$^{53}$, Y.~Pan$^{55}$, A.~~Pathak$^{33}$, Y.~P.~Pei$^{69,56}$, M.~Pelizaeus$^{4}$, H.~P.~Peng$^{69,56}$, K.~Peters$^{14,d}$, J.~L.~Ping$^{40}$, R.~G.~Ping$^{1,61}$, S.~Plura$^{34}$, S.~Pogodin$^{35}$, V.~Prasad$^{32}$, F.~Z.~Qi$^{1}$, H.~Qi$^{69,56}$, H.~R.~Qi$^{59}$, M.~Qi$^{41}$, T.~Y.~Qi$^{12,f}$, S.~Qian$^{1,56}$, W.~B.~Qian$^{61}$, C.~F.~Qiao$^{61}$, J.~J.~Qin$^{70}$, L.~Q.~Qin$^{15}$, X.~P.~Qin$^{12,f}$, X.~S.~Qin$^{48}$, Z.~H.~Qin$^{1,56}$, J.~F.~Qiu$^{1}$, S.~Q.~Qu$^{59}$, C.~F.~Redmer$^{34}$, K.~J.~Ren$^{38}$, A.~Rivetti$^{72C}$, V.~Rodin$^{62}$, M.~Rolo$^{72C}$, G.~Rong$^{1,61}$, Ch.~Rosner$^{19}$, S.~N.~Ruan$^{42}$, N.~Salone$^{43}$, A.~Sarantsev$^{35,c}$, Y.~Schelhaas$^{34}$, K.~Schoenning$^{73}$, M.~Scodeggio$^{29A,29B}$, K.~Y.~Shan$^{12,f}$, W.~Shan$^{24}$, X.~Y.~Shan$^{69,56}$, J.~F.~Shangguan$^{53}$, L.~G.~Shao$^{1,61}$, M.~Shao$^{69,56}$, C.~P.~Shen$^{12,f}$, H.~F.~Shen$^{1,61}$, W.~H.~Shen$^{61}$, X.~Y.~Shen$^{1,61}$, B.~A.~Shi$^{61}$, H.~C.~Shi$^{69,56}$, J.~L.~Shi$^{12}$, J.~Y.~Shi$^{1}$, Q.~Q.~Shi$^{53}$, R.~S.~Shi$^{1,61}$, X.~Shi$^{1,56}$, J.~J.~Song$^{20}$, T.~Z.~Song$^{57}$, W.~M.~Song$^{33,1}$, Y. ~J.~Song$^{12}$, Y.~X.~Song$^{45,g}$, S.~Sosio$^{72A,72C}$, S.~Spataro$^{72A,72C}$, F.~Stieler$^{34}$, Y.~J.~Su$^{61}$, G.~B.~Sun$^{74}$, G.~X.~Sun$^{1}$, H.~Sun$^{61}$, H.~K.~Sun$^{1}$, J.~F.~Sun$^{20}$, K.~Sun$^{59}$, L.~Sun$^{74}$, S.~S.~Sun$^{1,61}$, T.~Sun$^{1,61}$, W.~Y.~Sun$^{33}$, Y.~Sun$^{9}$, Y.~J.~Sun$^{69,56}$, Y.~Z.~Sun$^{1}$, Z.~T.~Sun$^{48}$, Y.~X.~Tan$^{69,56}$, C.~J.~Tang$^{52}$, G.~Y.~Tang$^{1}$, J.~Tang$^{57}$, Y.~A.~Tang$^{74}$, L.~Y~Tao$^{70}$, Q.~T.~Tao$^{25,h}$, M.~Tat$^{67}$, J.~X.~Teng$^{69,56}$, V.~Thoren$^{73}$, W.~H.~Tian$^{57}$, W.~H.~Tian$^{50}$, Y.~Tian$^{30,61}$, Z.~F.~Tian$^{74}$, I.~Uman$^{60B}$, B.~Wang$^{1}$, B.~L.~Wang$^{61}$, Bo~Wang$^{69,56}$, C.~W.~Wang$^{41}$, D.~Y.~Wang$^{45,g}$, F.~Wang$^{70}$, H.~J.~Wang$^{37,j,k}$, H.~P.~Wang$^{1,61}$, K.~Wang$^{1,56}$, L.~L.~Wang$^{1}$, M.~Wang$^{48}$, Meng~Wang$^{1,61}$, S.~Wang$^{12,f}$, S.~Wang$^{37,j,k}$, T. ~Wang$^{12,f}$, T.~J.~Wang$^{42}$, W. ~Wang$^{70}$, W.~Wang$^{57}$, W.~H.~Wang$^{74}$, W.~P.~Wang$^{69,56}$, X.~Wang$^{45,g}$, X.~F.~Wang$^{37,j,k}$, X.~J.~Wang$^{38}$, X.~L.~Wang$^{12,f}$, Y.~Wang$^{59}$, Y.~D.~Wang$^{44}$, Y.~F.~Wang$^{1,56,61}$, Y.~H.~Wang$^{46}$, Y.~N.~Wang$^{44}$, Y.~Q.~Wang$^{1}$, Yaqian~Wang$^{18,1}$, Yi~Wang$^{59}$, Z.~Wang$^{1,56}$, Z.~L. ~Wang$^{70}$, Z.~Y.~Wang$^{1,61}$, Ziyi~Wang$^{61}$, D.~Wei$^{68}$, D.~H.~Wei$^{15}$, F.~Weidner$^{66}$, S.~P.~Wen$^{1}$, C.~W.~Wenzel$^{4}$, U.~Wiedner$^{4}$, G.~Wilkinson$^{67}$, M.~Wolke$^{73}$, L.~Wollenberg$^{4}$, C.~Wu$^{38}$, J.~F.~Wu$^{1,61}$, L.~H.~Wu$^{1}$, L.~J.~Wu$^{1,61}$, X.~Wu$^{12,f}$, X.~H.~Wu$^{33}$, Y.~Wu$^{69}$, Y.~J~Wu$^{30}$, Z.~Wu$^{1,56}$, L.~Xia$^{69,56}$, X.~M.~Xian$^{38}$, T.~Xiang$^{45,g}$, D.~Xiao$^{37,j,k}$, G.~Y.~Xiao$^{41}$, H.~Xiao$^{12,f}$, S.~Y.~Xiao$^{1}$, Y. ~L.~Xiao$^{12,f}$, Z.~J.~Xiao$^{40}$, C.~Xie$^{41}$, X.~H.~Xie$^{45,g}$, Y.~Xie$^{48}$, Y.~G.~Xie$^{1,56}$, Y.~H.~Xie$^{6}$, Z.~P.~Xie$^{69,56}$, T.~Y.~Xing$^{1,61}$, C.~F.~Xu$^{1,61}$, C.~J.~Xu$^{57}$, G.~F.~Xu$^{1}$, H.~Y.~Xu$^{64}$, Q.~J.~Xu$^{17}$, W.~L.~Xu$^{64}$, X.~P.~Xu$^{53}$, Y.~C.~Xu$^{76}$, Z.~P.~Xu$^{41}$, F.~Yan$^{12,f}$, L.~Yan$^{12,f}$, W.~B.~Yan$^{69,56}$, W.~C.~Yan$^{79}$, X.~Q~Yan$^{1}$, H.~J.~Yang$^{49,e}$, H.~L.~Yang$^{33}$, H.~X.~Yang$^{1}$, Tao~Yang$^{1}$, Y.~Yang$^{12,f}$, Y.~F.~Yang$^{42}$, Y.~X.~Yang$^{1,61}$, Yifan~Yang$^{1,61}$, Z.~W.~Yang$^{37,j,k}$, M.~Ye$^{1,56}$, M.~H.~Ye$^{8}$, J.~H.~Yin$^{1}$, Z.~Y.~You$^{57}$, B.~X.~Yu$^{1,56,61}$, C.~X.~Yu$^{42}$, G.~Yu$^{1,61}$, T.~Yu$^{70}$, X.~D.~Yu$^{45,g}$, C.~Z.~Yuan$^{1,61}$, L.~Yuan$^{2}$, S.~C.~Yuan$^{1}$, X.~Q.~Yuan$^{1}$, Y.~Yuan$^{1,61}$, Z.~Y.~Yuan$^{57}$, C.~X.~Yue$^{38}$, A.~A.~Zafar$^{71}$, F.~R.~Zeng$^{48}$, X.~Zeng$^{12,f}$, Y.~Zeng$^{25,h}$, Y.~J.~Zeng$^{1,61}$, X.~Y.~Zhai$^{33}$, Y.~H.~Zhan$^{57}$, A.~Q.~Zhang$^{1,61}$, B.~L.~Zhang$^{1,61}$, B.~X.~Zhang$^{1}$, D.~H.~Zhang$^{42}$, G.~Y.~Zhang$^{20}$, H.~Zhang$^{69}$, H.~H.~Zhang$^{57}$, H.~H.~Zhang$^{33}$, H.~Q.~Zhang$^{1,56,61}$, H.~Y.~Zhang$^{1,56}$, J.~J.~Zhang$^{50}$, J.~L.~Zhang$^{75}$, J.~Q.~Zhang$^{40}$, J.~W.~Zhang$^{1,56,61}$, J.~X.~Zhang$^{37,j,k}$, J.~Y.~Zhang$^{1}$, J.~Z.~Zhang$^{1,61}$, Jiawei~Zhang$^{1,61}$, L.~M.~Zhang$^{59}$, L.~Q.~Zhang$^{57}$, Lei~Zhang$^{41}$, P.~Zhang$^{1}$, Q.~Y.~~Zhang$^{38,79}$, Shuihan~Zhang$^{1,61}$, Shulei~Zhang$^{25,h}$, X.~D.~Zhang$^{44}$, X.~M.~Zhang$^{1}$, X.~Y.~Zhang$^{53}$, X.~Y.~Zhang$^{48}$, Y.~Zhang$^{67}$, Y. ~T.~Zhang$^{79}$, Y.~H.~Zhang$^{1,56}$, Yan~Zhang$^{69,56}$, Yao~Zhang$^{1}$, Z.~H.~Zhang$^{1}$, Z.~L.~Zhang$^{33}$, Z.~Y.~Zhang$^{74}$, Z.~Y.~Zhang$^{42}$, G.~Zhao$^{1}$, J.~Zhao$^{38}$, J.~Y.~Zhao$^{1,61}$, J.~Z.~Zhao$^{1,56}$, Lei~Zhao$^{69,56}$, Ling~Zhao$^{1}$, M.~G.~Zhao$^{42}$, S.~J.~Zhao$^{79}$, Y.~B.~Zhao$^{1,56}$, Y.~X.~Zhao$^{30,61}$, Z.~G.~Zhao$^{69,56}$, A.~Zhemchugov$^{35,a}$, B.~Zheng$^{70}$, J.~P.~Zheng$^{1,56}$, W.~J.~Zheng$^{1,61}$, Y.~H.~Zheng$^{61}$, B.~Zhong$^{40}$, X.~Zhong$^{57}$, H. ~Zhou$^{48}$, L.~P.~Zhou$^{1,61}$, X.~Zhou$^{74}$, X.~K.~Zhou$^{6}$, X.~R.~Zhou$^{69,56}$, X.~Y.~Zhou$^{38}$, Y.~Z.~Zhou$^{12,f}$, J.~Zhu$^{42}$, K.~Zhu$^{1}$, K.~J.~Zhu$^{1,56,61}$, L.~Zhu$^{33}$, L.~X.~Zhu$^{61}$, S.~H.~Zhu$^{68}$, S.~Q.~Zhu$^{41}$, T.~J.~Zhu$^{12,f}$, W.~J.~Zhu$^{12,f}$, Y.~C.~Zhu$^{69,56}$, Z.~A.~Zhu$^{1,61}$, J.~H.~Zou$^{1}$, J.~Zu$^{69,56}$
\\
\vspace{0.2cm}
(BESIII Collaboration)\\
\vspace{0.2cm} {\it
$^{1}$ Institute of High Energy Physics, Beijing 100049, People's Republic of China\\
$^{2}$ Beihang University, Beijing 100191, People's Republic of China\\
$^{3}$ Beijing Institute of Petrochemical Technology, Beijing 102617, People's Republic of China\\
$^{4}$ Bochum  Ruhr-University, D-44780 Bochum, Germany\\
$^{5}$ Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, USA\\
$^{6}$ Central China Normal University, Wuhan 430079, People's Republic of China\\
$^{7}$ Central South University, Changsha 410083, People's Republic of China\\
$^{8}$ China Center of Advanced Science and Technology, Beijing 100190, People's Republic of China\\
$^{9}$ China University of Geosciences, Wuhan 430074, People's Republic of China\\
$^{10}$ Chung-Ang University, Seoul, 06974, Republic of Korea\\
$^{11}$ COMSATS University Islamabad, Lahore Campus, Defence Road, Off Raiwind Road, 54000 Lahore, Pakistan\\
$^{12}$ Fudan University, Shanghai 200433, People's Republic of China\\
$^{13}$ G.I. Budker Institute of Nuclear Physics SB RAS (BINP), Novosibirsk 630090, Russia\\
$^{14}$ GSI Helmholtzcentre for Heavy Ion Research GmbH, D-64291 Darmstadt, Germany\\
$^{15}$ Guangxi Normal University, Guilin 541004, People's Republic of China\\
$^{16}$ Guangxi University, Nanning 530004, People's Republic of China\\
$^{17}$ Hangzhou Normal University, Hangzhou 310036, People's Republic of China\\
$^{18}$ Hebei University, Baoding 071002, People's Republic of China\\
$^{19}$ Helmholtz Institute Mainz, Staudinger Weg 18, D-55099 Mainz, Germany\\
$^{20}$ Henan Normal University, Xinxiang 453007, People's Republic of China\\
$^{21}$ Henan University of Science and Technology, Luoyang 471003, People's Republic of China\\
$^{22}$ Henan University of Technology, Zhengzhou 450001, People's Republic of China\\
$^{23}$ Huangshan College, Huangshan  245000, People's Republic of China\\
$^{24}$ Hunan Normal University, Changsha 410081, People's Republic of China\\
$^{25}$ Hunan University, Changsha 410082, People's Republic of China\\
$^{26}$ Indian Institute of Technology Madras, Chennai 600036, India\\
$^{27}$ Indiana University, Bloomington, Indiana 47405, USA\\
$^{28}$ INFN Laboratori Nazionali di Frascati , (A)INFN Laboratori Nazionali di Frascati, I-00044, Frascati, Italy; (B)INFN Sezione di  Perugia, I-06100, Perugia, Italy; (C)University of Perugia, I-06100, Perugia, Italy\\
$^{29}$ INFN Sezione di Ferrara, (A)INFN Sezione di Ferrara, I-44122, Ferrara, Italy; (B)University of Ferrara,  I-44122, Ferrara, Italy\\
$^{30}$ Institute of Modern Physics, Lanzhou 730000, People's Republic of China\\
$^{31}$ Institute of Physics and Technology, Peace Avenue 54B, Ulaanbaatar 13330, Mongolia\\
$^{32}$ Instituto de Alta Investigaci\'on, Universidad de Tarapac\'a, Casilla 7D, Arica, Chile\\
$^{33}$ Jilin University, Changchun 130012, People's Republic of China\\
$^{34}$ Johannes Gutenberg University of Mainz, Johann-Joachim-Becher-Weg 45, D-55099 Mainz, Germany\\
$^{35}$ Joint Institute for Nuclear Research, 141980 Dubna, Moscow region, Russia\\
$^{36}$ Justus-Liebig-Universitaet Giessen, II. Physikalisches Institut, Heinrich-Buff-Ring 16, D-35392 Giessen, Germany\\
$^{37}$ Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{38}$ Liaoning Normal University, Dalian 116029, People's Republic of China\\
$^{39}$ Liaoning University, Shenyang 110036, People's Republic of China\\
$^{40}$ Nanjing Normal University, Nanjing 210023, People's Republic of China\\
$^{41}$ Nanjing University, Nanjing 210093, People's Republic of China\\
$^{42}$ Nankai University, Tianjin 300071, People's Republic of China\\
$^{43}$ National Centre for Nuclear Research, Warsaw 02-093, Poland\\
$^{44}$ North China Electric Power University, Beijing 102206, People's Republic of China\\
$^{45}$ Peking University, Beijing 100871, People's Republic of China\\
$^{46}$ Qufu Normal University, Qufu 273165, People's Republic of China\\
$^{47}$ Shandong Normal University, Jinan 250014, People's Republic of China\\
$^{48}$ Shandong University, Jinan 250100, People's Republic of China\\
$^{49}$ Shanghai Jiao Tong University, Shanghai 200240,  People's Republic of China\\
$^{50}$ Shanxi Normal University, Linfen 041004, People's Republic of China\\
$^{51}$ Shanxi University, Taiyuan 030006, People's Republic of China\\
$^{52}$ Sichuan University, Chengdu 610064, People's Republic of China\\
$^{53}$ Soochow University, Suzhou 215006, People's Republic of China\\
$^{54}$ South China Normal University, Guangzhou 510006, People's Republic of China\\
$^{55}$ Southeast University, Nanjing 211100, People's Republic of China\\
$^{56}$ State Key Laboratory of Particle Detection and Electronics, Beijing 100049, Hefei 230026, People's Republic of China\\
$^{57}$ Sun Yat-Sen University, Guangzhou 510275, People's Republic of China\\
$^{58}$ Suranaree University of Technology, University Avenue 111, Nakhon Ratchasima 30000, Thailand\\
$^{59}$ Tsinghua University, Beijing 100084, People's Republic of China\\
$^{60}$ Turkish Accelerator Center Particle Factory Group, (A)Istinye University, 34010, Istanbul, Turkey; (B)Near East University, Nicosia, North Cyprus, 99138, Mersin 10, Turkey\\
$^{61}$ University of Chinese Academy of Sciences, Beijing 100049, People's Republic of China\\
$^{62}$ University of Groningen, NL-9747 AA Groningen, The Netherlands\\
$^{63}$ University of Hawaii, Honolulu, Hawaii 96822, USA\\
$^{64}$ University of Jinan, Jinan 250022, People's Republic of China\\
$^{65}$ University of Manchester, Oxford Road, Manchester, M13 9PL, United Kingdom\\
$^{66}$ University of Muenster, Wilhelm-Klemm-Strasse 9, 48149 Muenster, Germany\\
$^{67}$ University of Oxford, Keble Road, Oxford OX13RH, United Kingdom\\
$^{68}$ University of Science and Technology Liaoning, Anshan 114051, People's Republic of China\\
$^{69}$ University of Science and Technology of China, Hefei 230026, People's Republic of China\\
$^{70}$ University of South China, Hengyang 421001, People's Republic of China\\
$^{71}$ University of the Punjab, Lahore-54590, Pakistan\\
$^{72}$ University of Turin and INFN, (A)University of Turin, I-10125, Turin, Italy; (B)University of Eastern Piedmont, I-15121, Alessandria, Italy; (C)INFN, I-10125, Turin, Italy\\
$^{73}$ Uppsala University, Box 516, SE-75120 Uppsala, Sweden\\
$^{74}$ Wuhan University, Wuhan 430072, People's Republic of China\\
$^{75}$ Xinyang Normal University, Xinyang 464000, People's Republic of China\\
$^{76}$ Yantai University, Yantai 264005, People's Republic of China\\
$^{77}$ Yunnan University, Kunming 650500, People's Republic of China\\
$^{78}$ Zhejiang University, Hangzhou 310027, People's Republic of China\\
$^{79}$ Zhengzhou University, Zhengzhou 450001, People's Republic of China\\
\vspace{0.2cm}
$^{a}$ Also at the Moscow Institute of Physics and Technology, Moscow 141700, Russia\\
$^{b}$ Also at the Novosibirsk State University, Novosibirsk, 630090, Russia\\
$^{c}$ Also at the NRC "Kurchatov Institute", PNPI, 188300, Gatchina, Russia\\
$^{d}$ Also at Goethe University Frankfurt, 60323 Frankfurt am Main, Germany\\
$^{e}$ Also at Key Laboratory for Particle Physics, Astrophysics and Cosmology, Ministry of Education; Shanghai Key Laboratory for Particle Physics and Cosmology; Institute of Nuclear and Particle Physics, Shanghai 200240, People's Republic of China\\
$^{f}$ Also at Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443, People's Republic of China\\
$^{g}$ Also at State Key Laboratory of Nuclear Physics and Technology, Peking University, Beijing 100871, People's Republic of China\\
$^{h}$ Also at School of Physics and Electronics, Hunan University, Changsha 410082, China\\
$^{i}$ Also at Guangdong Provincial Key Laboratory of Nuclear Science, Institute of Quantum Matter, South China Normal University, Guangzhou 510006, China\\
$^{j}$ Also at Frontiers Science Center for Rare Isotopes, Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{k}$ Also at Lanzhou Center for Theoretical Physics, Lanzhou University, Lanzhou 730000, People's Republic of China\\
$^{l}$ Also at the Department of Mathematical Sciences, IBA, Karachi , Pakistan\\
}\vspace{0.4cm}  }  
%% ends here %%

